An Approach for Detecting Dynamic Communities in Social Networks

Recent developments in the internet and technology have made major advancements in tools that facilitate the collection of social data, opening up thus new opportunities for analyzing social networks. Social network analysis studies the patterns of social relations and aims at discovering the hidden features embedded in the structure of social networks. One of the most important features in social networks is community structure : densely knit groups of individuals. The dynamic nature of interaction in social networks often challenges the detection of such community structures. The contributions in this thesis fall into two categories.The first category highlights the problem of identifying overlapping communities over time. To carry out such analysis, a framework called OLCPM (Online Label propagation and Clique Percolation Method) is proposed. It is an online algorithm based on clique percolation and label propagation methods. OLCPM has two main features : the first one is its ability to discover overlapping communities, while the second is its effectiveness in handling fine-grained temporal net works. As for as the second category is concerned, it emphasizes on the problem of analyzing communities that are embedded at different temporal scales. For example, in networks of interaction such as e-mails or phone calls, individuals are involved in daily as well as occasional conversations. We propose a first method for analyzing communities at multiple temporal scales. Hence, the dynamic network (link streams) is studied at different temporal granularities, and coherent communities (called stable communities) over a period of time are detected at each temporal granularity. The two proposed approaches are validated on both synthetic and real-world datasets.

==> Chapters/xxx.tex <==
\section{Introduction}
In recent years, studying interactions over time has witnessed a growing interest in a wide range of fields, such as sociology, biology, physics, etc. Such dynamic interactions are often represented using the snapshot model: the network is divided into a sequence of static networks, i.e., snapshots, aggregating all contacts occurring in a given time window. The main drawback of this model is that it often requires to choose arbitrarily a temporal scale of analysis. The link stream model \cite{Latapy2018} is a more effective way for representing interactions over time, that can fully capture the underlying temporal information. Under this model, the main challenge is to mine more efficiently and smoothly both temporal and topological structures. 

Real-world networks evolve frequently at many different time scales. Fluctuations in such networks can be observed at yearly, monthly, daily, hourly, or even smaller scales.  For instance, if one were to look at interactions among workers in a company or laboratory, one could expect to discover clusters of people corresponding to \textit{meetings} and/or \textit{coffee breaks}, interacting at \textbf{high frequency} (e.g., every few seconds) for \textbf{short periods} (e.g., few minutes), \textit{project members} interacting at medium frequency (e.g., once a day) for medium periods (e.g., a few months), \textit{coordination groups} interacting at low frequency (e.g., once a month) for longer periods (e.g., a few years), etc.

An analysis of communities found at an arbitrarily chosen scale would necessarily miss some of these communities: low latency ones are invisible using short aggregation windows, while high-frequency ones are lost in the noise for long aggregation windows. A multiple temporal scale analysis of communities seems therefore the right solution to study networks of interactions represented as link streams.

To the best of our knowledge, no such method exists in the literature. In this chapter, we propose a method having roots both in the literature in dynamic community detection and in change-point detection. The aim of the former is to discover groups that persist overtime , while the objective of the latter is to detect changes in the overall structure of a dynamic network. %It detects what we call \textbf{stable communities}, i.e., \textit{groups of nodes} forming a \textit{coherent community} throughout a \textit{period of time}, at a given \textit{temporal scale}. %The proposed method falls into the class of Cross-time approaches. 

Most dynamic community detection methods consider that the studied dynamic networks are represented as sequences of snapshots, with each snapshot being a well-formed graph with meaningful community structure, see for instance \cite{mucha2010community,greene2010tracking}. Some other methods work with interval graphs and update the community structure at each network change, e.g., \cite{rossetti2017tiles,boudebza2018}, or by searching dense sub-graphs \cite{gaumont2016finding}. However, those methods are not adapted to deal with link streams, for which the network is usually not well-formed at any given time. Using them on such a network would require to first aggregate the links of the stream by choosing arbitrarily a temporal scale (aggregation window). A few methods exist nevertheless to handle link streams: In \cite{Viard:2016:CMC:2853249.2853730}, Viand and Latapy introduced a method to discover efficiently maximal $\Delta$ cliques in link streams, i.e., groups of nodes having at least one interaction between all of them during a user-defined period $\Delta$. Note that this method is limited to the detection of cliques, an extreme case of communities. It also requires to fix a unique granularity using a time period $\Delta$. In \cite{matias2017statistical}, a method based on stochastic block models is proposed by Matias and Miele. Its principle is to discover groups of nodes that interact similarly between themselves or with other groups of nodes during one or several periods of time, without constraint on the frequency of those interactions, but only on their similarity. A limit of this work is that it is able to find a single partition of the nodes, that is considered constant through time. It is therefore impossible for nodes to switch between communities, appear, disappear or change behaviors. Compared to those methods, the solution we propose is able to: $i)$ Discover communities at multiple temporal scales without redundancy and $ii)$ Allow nodes to belong to several communities, at different periods and different temporal scales.

Our work is also related to research conducted on change-point detection considering community structures in dynamic networks. 
In these approaches, given a sequence of snapshots, one wants to detect periods during which the network organization and/or the community structure remains stable. 
\cite{Peel204} proposed the first change-point detection method for evolving networks that uses generative network models and statistical hypothesis testing. The Generalized Hierarchical Random Graph (GHRG) model is used to define a parametric probability distribution over network snapshots and to compactly model nested community structure. Then, two models are inferred (a model for representing the change at time $t$ in the snapshot, and a model for representing the null hypothesis of no change over the entire snapshot). Bayesian hypothesis testing is used to choose the best model. This method can detect when do the change occurs, and the shape of the change. The main issue of this method is its scalability on large networks. 
\cite{Wang2017} proposed a method to detect local and global change points in the community structure. Each snapshot is contracted into a weighted hypergraph, in which hyper-nodes are the communities detected at this snapshot. Then, local changes are detected by measuring similarities between hyper-nodes (communities) in successive hyper-networks, while global changes are detected by running community detection algorithms on successive hyper-graphs. 
Similarly, \cite{Zhu2018} formulated the problem of change point detection as clustering of hyper-networks. %in \cite{Zhu2018} the problem of change point detection is formulated as a clustering of hyper-networks. 
First, they construct a weighted hyper-network, where nodes represent the snapshots and weights represent similarities between snapshots, based on structural feature and similarity measurements (relative importance of nodes). Then, community detection is run on this hyper-graph. At final, they serialize the community detection results in chronological order, where each snapshot is labeled by its community identity. This method can detect i)local changes, ii)global changes and iii)isomorphic changes.
We also note that our work is related to the one by \cite{Masuda2019}. The authors seek to identify sequences of system states in data streams. The idea is to i) transform a data stream into a sequence of snapshots (non-overlapping windows of size $W$), ii) measure the pairwise distance between snapshots, iii) run a clustering algorithm on the matrix distance and categorize snapshots into discrete states.
From those methods, our proposal keeps the principle of stable periods delimited by change points, and the idea of detecting changes at local and global scales. But our method differs in two directions: i) we are searching for stable individual communities instead of stable graph periods, and ii) we search for stable structures at multiple levels of temporal granularity.

%We share the full code of the proposed method and of the experimental process on a public repository\footnote{\url{https://github.com/Yquetzal/ECML_PKDD_2019}}, including an online notebook allowing to easily test the method with no set-up configuration\footnote{\url{https://colab.research.google.com/github/Yquetzal/ECML_PKDD_2019/blob/master/simple_demo.ipynb}}.

The remainder of this chapter is organized as follows. In Section \ref{framework}, we describe the proposed framework in detail. We experimentally evaluate the proposed method on both synthetic and real-world networks in Section \ref{experiments}.%%%%%%%%%%%
\begin{comment}
Gauvin et al. \cite{aynaud2011multi}& 
CT& 
{\textcolor{red}{SN}}& 
&
&
\\ \hline
Sarantopolos et al. \cite{sarantopoulos2018timerank}& 
CT& 
{\textcolor{red}{SN}}& 
&
&
\\ \hline
Yan et al. \cite{}& 
CT& 
{\textcolor{red}{SN}}& 
&
&
\\ \hline
\\ \hline
Guo et al. \cite{guo2014evolutionary}& 
TTO& 
{\textcolor{green!80!black}{TN}}& 
\xmark&
\xmark&
\xmark
\begin{itemize}
\item Some definitions are \textit{stochastic} and/or \textit{extrinsic}, and thus lead to two major problems:
Instability : This problem happens when different runs on the same (slightly modified) network lead to very different results. It affects only the two classes of Instant Optimal  approaches and Temporal Trade-off approaches which are based on stochastic and non deterministic community definitions, like those based on Modularity \cite{asur2009event}, or on random walk \cite{tajeuna2015tracking}. Cross time approaches don't suffer from the instability problem as they propose to study simultaneously all the network evolution steps. Diffrent solutions have been proposed to mitigate this problem : Hopcroft et al. \cite{hopcroft2004tracking} search  for invariant parts of the communities by performing multiple runs of the same algorithm on the same snapshot, Wang et al.\cite{wang2008community} used the concept of Community core nodes, Xu et al. \cite{xu2013analyzing,xu2013community} search for stable community core, Chen et al. \cite{chen2010detecting} use the notion of graph representatives and community representatives, Aynaud et Guillaume \cite{aynaud2010static} proposed a global optimization process in which the modularity is maximized on multiple snapshots rather than one snapshot, Chakrabrti el al. \cite{chakrabarti2006evolutionary} integrate the history cost in their objective function. Methods using deterministic definitions resolve naturally this problem, like k-clique community definition in the CPM method by Palla et al. \cite{palla2007quantifying}.
%Methods in the class of Cross Time approaches don’t suffer from this problem as well, as they consider simultaneously all the network evolution steps.
Community drifting effects: which means that the solution can be dragged away from an originally relevant solution. This problem my affects only temporal trade-off approaches, and more precisely, the updating approaches (see methods in \cite{aynaud2010static, nguyen2011adaptive,aktunc2015dynamic}), when communities at a time $t$ are computed by updating the ones discovered at previous time step $t-1$. Community drift phenomenon arises from the use of non-intrinsic community definitions, i.e., when the community definition depends on the whole network (like modularity), a community can be modified as a result of some changes in an unrelated part of the network, and this could lead to misleading results. It my also occurs when using stochastic community definitions, as partitions evolve based on local optimal solutions, it is not guaranteed to yield an optimal solution at the global level.

\item Most definitions are designed for \textit{disjoint} (non-overlapping) communities, i.e., a node cannot be part of several communities. The ability to detect an overlapping coverage is a crucial question in community detection, especially when exploring real world networks such as social networks. In such networks, nodes are likely belong to multiple communities, in an online social network for example, a member may be connected to co-workers, friends , family,  neighbors, etc. Few method are enable to detect such overlapping community structures, as example: CPM method \cite{palla2007quantifying} which use the concept of maximal k-clique, the method by  ... 
\end{itemize}

In this thesis we are particularly interested on highly dynamic social networks. Such networks has some peculiar characteristics.

Temporal networks: snapshot models cannot capture the \textit{\textbf{full temporal evolution}} of the networks, and hence methods based on this model (such as )are not suitable to deal with highly evolving networks, which is the case of most real world networks like social networks. On the contrary, temporal network is the appropriate model to deal with \textit{highly evolving networks}, but methods using such a model (like ) are \textit{computationally expensive}, as they require repetitive computations of communities at each network change. Therefore, the majority of recent methods adopts local computations to minimize the computational cost, like the method by Nguyen et al. \cite{nguyen2011adaptive}. 

The stability of detection is an important aspect to take into account  when dealing with very dynamic networks.
Instability : 
This problem affects only the two classes of Instant Optimal  approaches and Temporal Trade-off approaches which are based on stochastic and non deterministic community definitions, like those based on Modularity \cite{asur2009event}, or on random walk \cite{tajeuna2015tracking}. Cross time approaches don't suffer from the instability problem as they propose to study simultaneously all the network evolution steps. 
Different solutions have been proposed to mitigate this problem : Hopcroft et al. \cite{hopcroft2004tracking} search  for invariant parts of the communities by performing multiple runs of the same algorithm on the same snapshot, Wang et al.\cite{wang2008community} used the concept of Community core nodes, Xu et al. \cite{xu2013analyzing,xu2013community} search for stable community core, Chen et al. \cite{chen2010detecting} use the notion of graph representatives and community representatives, Aynaud et Guillaume \cite{aynaud2010static} proposed a global optimization process in which the modularity is maximized on multiple snapshots rather than one snapshot, Chakrabrti el al. \cite{chakrabarti2006evolutionary} integrate the history cost in their objective function. Methods using deterministic definitions resolve naturally this problem, like k-clique community definition in the CPM method by Palla et al. \cite{palla2007quantifying}.

The avalanche aspect or community drift problem. This problem my affects only temporal trade-off approaches, and more precisely, the updating approaches (see methods in \cite{aynaud2010static, nguyen2011adaptive,aktunc2015dynamic}). Community drift phenomenon arises from the use of non-intrinsic community definitions, i.e., when the community definition depends on the whole network (like modularity), a community can be modified as a result of some changes in an unrelated part of the network, and this could lead to misleading results. It my also occurs when using stochastic community definitions, as partitions evolve based on local optimal solutions, it is not guaranteed to yield an optimal solution at the global level.
social network are known to be highly overlapping, thus most methods in the literature are not adapted to the problem we want to tackle. The best known exception is the CPM method REF. However, this method is only designed to tackle static networks. In our first contribution, we will thus propose a variant of CPM working on temporal networks…

Multiple temporal scale of Analysis :The snapshot model often requires to choose an arbitrary \textit{\textbf{temporal scale}} to divide the network. Communities detected at such an arbitrary temporal granularity could lead to misleading results: communities resulting from high frequency interactions and short duration are invisible when considering large temporal scale (window time), while communities resulting from low frequency interactions and large duration are invisible using a fine temporal granularity. A multiple temporal scale analysis of communities seem therefore the right solution in such a case. To the best of our knowledge, this question has not yet been studied in the literature.

As we can see, the two methods we will propose must meet all these requirements. Our first method which is a variant of the CPM method working on temporal networks. This method don’t suffer from the instability and the community drift problems as the CPM definition is deterministic. It is enable to detect overlapping community structures.
Our second Cross-time method which also works on temporal networks. This method don’t suffer from the problems of instability and risk of avalanche as the network as all the network evolution steps are studied simultaneously.This method is the first to consider a multiple temporal scale analysis to detect community structures.


%From this review of the literature, we can highlight significant research gaps that still need to be addressed on the topic of dynamic community detection, especially when dealing with social networks. 

As illustrated in Table \ref{tab:meth0}, theses issues are particularly related to the definition of community and to the underling network model used. 

\textbf{\textit{Community definition.}} The existing methodologies propose different definitions of dynamic communities: 
\begin{enumerate}[(i)]
\item Some definitions are \textit{\textbf{stochastic}} and/or \textit{\textbf{extrinsic}}, and thus lead to two major problems:
\begin{itemize}
\item \textbf{\textit{Instability:} }This problem happens when different runs on the same (slightly modified) network lead to very different results. It affects only the two classes of Instant Optimal  approaches and Temporal Trade-off approaches which are based on stochastic and non-deterministic community definitions, like those based on Modularity \cite{asur2009event}, or random walks \cite{tajeuna2015tracking}. Cross time approaches (see methods in \cite{aynaud2011multi, xu2013analyzing, xu2013community, ludkin2018dynamic, jdidia2007communities, mucha2010community}) don't suffer from the instability problem as they propose to study simultaneously all the network evolution steps. Different solutions have been proposed to mitigate this problem: Hopcroft et al. \cite{hopcroft2004tracking} search  for invariant parts of the communities by performing multiple runs of the same algorithm on the same snapshot, Wang et al.\cite{wang2008community} used the concept of Community core nodes, Xu et al. \cite{xu2013analyzing,xu2013community} search for stable community core, Chen et al. \cite{chen2010detecting} use the notion of graph representatives and community representatives, Aynaud and Guillaume \cite{aynaud2010static} propose a global optimization process in which the modularity is maximized on multiple snapshots rather than one snapshot, Chakrabrti el al. \cite{chakrabarti2006evolutionary} integrate the history cost in their objective function. Methods using deterministic definitions resolve naturally this problem, like k-clique community definition in the CPM method by Palla et al. \cite{palla2007quantifying}.
%Methods in the class of Cross Time approaches don’t suffer from this problem as well, as they consider simultaneously all the network evolution steps.
\item \textbf{\textit{Community drifting effects:}} Community drifting means that the solution can be dragged away from an originally relevant solution. This problem might affects only temporal trade-off approaches, and more precisely, the updating approaches (see methods in \cite{aynaud2010static, nguyen2011adaptive,aktunc2015dynamic}), when communities at a time $t$ are computed by updating the ones discovered at previous time step $t-1$. Community drift phenomenon arises from the use of non-intrinsic community definitions, i.e., when the community definition depends on the whole network (like modularity), a community can be modified as a result of some changes in an unrelated part of the network, and this could lead to misleading results. It may also occurs when using stochastic community definitions, as partitions evolve based on local optimal solutions, it is not guaranteed to yield an optimal solution at the global level.
\end{itemize}
\item Most definitions are designed for \textit{\textbf{disjoint}} (non-overlapping) communities, i.e., a node cannot be part of several communities. The ability to detect an overlapping coverage is a crucial question in community detection, especially when exploring real world networks such as social networks. In such networks, nodes are likely belonging to multiple communities, in an online social network for example, a member may be connected to co-workers, friends , family,  neighbors, etc. Few method are enable to detect such overlapping community structures, as example: CPM method \cite{palla2007quantifying} which use the concept of maximal k-clique, the method by  ... 
\end{enumerate}

\textbf{\textit{Network model.}} The way to model the network evolution is extremely important and it highly influence the community detection:

\begin{enumerate}[(i)] 
\item Snapshot models cannot capture the \textit{\textbf{full temporal evolution}} of the networks, and hence methods based on this model (such as )are not suitable to deal with highly evolving networks, which is the case of most real world networks like social networks. On the contrary, temporal network is the appropriate model to deal with \textit{highly evolving networks}, but methods using such a model(like ) are \textit{computationally expensive}, as they require repetitive computations of communities at each network change. Therefore, the majority of recent methods adopts local computations to minimize the computational cost, like the method by Nguyen et al. \cite{nguyen2011adaptive}.   
\item The snapshot model often requires to choose an arbitrary \textit{\textbf{temporal scale}} to divide the network. Communities detected at such an arbitrary temporal granularity could lead to misleading results: communities resulting from high frequency interactions and short duration are invisible when considering large temporal scale (window time), while communities resulting from low frequency interactions and large duration are invisible using a fine temporal granularity. A multiple temporal scale analysis of communities seem therefore the right solution in such a case. To the best of our knowledge, this question has not yet been studied in the literature.
\end{enumerate}
\subsection{Advantages and drawbacks of dynamic community detection approaches}

This classification highlights a variety of methods which propose different ways for solving the same problem and also different definitions of dynamic communities. %Despite the wide range of definitions and techniques proposed, there are still many 

The proposed taxonomy gives us some hints to choose the appropriate method. The choice depends on the purpose of the analysis. %As mentioned earlier, each classes has its own advantages and disadvantages and each of them is appropriated for a specific use case. 
For example, Instant-optimal approaches are the best choice %when dealing with less evolving networks or 
when the goal is to find communities of high quality at each time step. Temporal trad-off approaches are suitable for the online monitoring and tracking of communities. Finally, the Cross-time approaches are the best choice when the goal is to find coherent communities over a long period of time.



%As mentioned throughout this section, the three classes have their own advantages and disadvantages, and none of these classes is superior to the others. However, some criteria can be also considered while choosing the appropriate approach, like, the network model, instability and community drift problems, the  temporal complexity of the method, etc. 

\subsection{Positioning our contributions with respect to the state of the art}\label{chp3:Discussion}

From this review of the literature, we can highlight significant research gaps that still need to be addressed on the topic of dynamic community detection, especially when dealing with social networks. In this section, we will show how our contributions are the answer to the issues we have observed in this review. 
To do so, we use Table \ref{tab:meth0} which summarizes the comparison between methods of DCD. %The comparison is restricted to only methods designed for detecting overlapping community structures and generic methods which can be applied for both overlapping and  disjoint communities. 
Given the large number of methods being presented in this survey, the comparison is restricted to only some representative methods from each class of approaches. The following comparison criteria are used here:
\begin{itemize}
\item \textit{Approach:} indicates the class of approaches to which the method belongs: \textbf{IO} (Instant Optimal), \textbf{TTO} (Temporal Trade-off) or \textbf{CT} (CrossTime). 
\item Network model: refers to the type of the dynamic network model used by the method: {\textcolor{red}{SN}} (Snapshot Network), {\textcolor{green!80!black}{TN}} (Temporal networks).
\item \textit{Stability:} indicates if the method suffer (\xmark) or not (\cmark) from the Instability problem.
\item \textit{Avalanche safety :} %No community drift
indicates if the method suffer (\xmark) or not (\cmark) from the community drift problem.
\item \textit{Overlapping: }indicates it the method can detect overlapping community structures (\cmark) or not (\xmark).
\item \textit{Multi-temporal scale: }indicates it the method can detect community structures at multiple temporal scale (\cmark) or only on one temporal scale(\xmark).
\end{itemize}

\begin{table}[H]
\resizebox{\textwidth}{!}{%
%\small
\tiny
\begin{tabular}{|p{3.3cm}||p{1.4cm}|p{1.2cm}|p{1.3cm}|p{1.6cm}|p{1.7cm}|p{1.7cm}|}
\hline
\textbf{Reference} & \textbf{Approach}& \textbf{Network Model}& \textbf{Instability}& \textbf{Community drift}& \textbf{Overlapping}& \textbf{Multi-temporal scale} \\ \hline
Asur et al.\cite{asur2009event}& 
\textbf{IO}& 
\textbf{{\textcolor{red}{SN}}}& 
\xmark&
\cmark&
\xmark&
\xmark
\\ \hline
Hopcroft et al.\cite{hopcroft2004tracking}& 
\textbf{IO}& 
\textbf{{\textcolor{red}{SN}}}& 
\cmark&
\cmark&
\xmark&
\xmark
\\ \hline
Palla et al.\cite{palla2007quantifying}& 
\textbf{IO}& 
\textbf{{\textcolor{red}{SN}}}& 
\cmark&
\cmark&
\cmark&
\xmark
\\ \hline
Tajeuna et al.\cite{tajeuna2015tracking}& 
\textbf{IO}& 
\textbf{{\textcolor{red}{SN}}}& 
\xmark&
\cmark&
\xmark&
\xmark
\\ \hline
Wang et al.\cite{wang2008community}& 
\textbf{IO}& 
\textbf{{\textcolor{red}{SN}}}& 
\cmark&
\cmark&
\xmark&
\xmark
\\ \hline
Chen et al.\cite{chen2010detecting}& 
\textbf{IO}& 
\textbf{{\textcolor{red}{SN}}}& 
\cmark&
\cmark&
\xmark&
\xmark
\\ \hline
Aynaud and Guillaume \cite{aynaud2010static}& 
\textbf{TTO}& 
\textbf{{\textcolor{red}{SN}}}& 
\xmark&
\xmark&
\xmark&
\xmark
\\ \hline
Aktunc et al. \cite{aktunc2015dynamic}& 
\textbf{TTO}& 
\textbf{{\textcolor{red}{SN}}}& 
\xmark&
\xmark&
\xmark&
\xmark
\\ \hline
Nguyen et al. \cite{nguyen2011adaptive}& 
\textbf{TTO}& 
\textbf{{\textcolor{green!80!black}{TN}}}& 
\xmark&
\xmark&
\xmark&
\xmark
\\ \hline
Chakraborti et al. \cite{chakrabarti2006evolutionary}& 
\textbf{TTO}& 
\textbf{{\textcolor{red}{SN}}}& 
\cmark&
\xmark&
\xmark&
\xmark
\\ \hline
Xu et al. \cite{xu2013analyzing,xu2013community}& 
\textbf{TTO}& 
{{\textcolor{green!80!black}{TN}}}&%\textbf{{\textcolor{red}{SN}}}& 
\cmark&
\xmark&
\xmark&
\xmark
\\ \hline
Aynaud et Guillaume \cite{aynaud2011multi}& 
\textbf{CT}& 
\textbf{{\textcolor{red}{SN}}}& 
\cmark&
\cmark&
\xmark&
\xmark
\\ \hline
Xu et al. \cite{xu2013analyzing,xu2013community}& 
\textbf{CT}& 
\textbf{{\textcolor{red}{SN}}}& 
\cmark&
\cmark&
\xmark&
\xmark
\\ \hline
Ludkin et al. \cite{ludkin2018dynamic}& 
\textbf{CT}& 
\textbf{{\textcolor{red}{SN}}}& 
\cmark&
\cmark&
\xmark&
\xmark
\\ \hline
Mucha et al. \cite{mucha2010community}& 
\textbf{CT}& 
\textbf{{\textcolor{red}{SN}}}& 
\cmark&
\cmark&
\xmark&
\xmark
\\ \hline
Jdidia et al. \cite{jdidia2007communities}& 
\textbf{CT}& 
\textbf{{\textcolor{red}{SN}}}& 
\cmark&
\cmark&
\xmark&
\xmark
\\ \hline
\textbf{Our $1^{st}$ method \cite{boudebza2018}}& 
\textbf{TTO}& 
\textbf{{\textcolor{green!80!black}{TN}}}& 
\cmark&
\cmark&
\cmark&
\xmark
\\ \hline
\textbf{Our $2^{nd}$  method \cite{boudebza2019detecting}}& 
\textbf{CT}& 
\textbf{{\textcolor{green!80!black}{TN}}}& 
\cmark&
\cmark&
\cmark&
\cmark
\\ \hline
\end{tabular}}
\caption{Comparing dynamic community detection methods.}
\label{tab:meth0}
\end{table}

Gauvin et al. \cite{aynaud2011multi}& 
CT& 
{\textcolor{red}{SN}}& 
&
&
\\ \hline
Sarantopolos et al. \cite{sarantopoulos2018timerank}& 
CT& 
{\textcolor{red}{SN}}& 
&
&
\\ \hline
Yan et al. \cite{}& 
CT& 
{\textcolor{red}{SN}}& 
&
&
\\ \hline
\\ \hline
Guo et al. \cite{guo2014evolutionary}& 
TTO& 
{\textcolor{green!80!black}{TN}}& 
\xmark&
\xmark&
\xmark
\begin{itemize}
\item Some definitions are \textit{stochastic} and/or \textit{extrinsic}, and thus lead to two major problems:
Instability : This problem happens when different runs on the same (slightly modified) network lead to very different results. It affects only the two classes of Instant Optimal  approaches and Temporal Trade-off approaches which are based on stochastic and non deterministic community definitions, like those based on Modularity \cite{asur2009event}, or on random walk \cite{tajeuna2015tracking}. Cross time approaches don't suffer from the instability problem as they propose to study simultaneously all the network evolution steps. Diffrent solutions have been proposed to mitigate this problem : Hopcroft et al. \cite{hopcroft2004tracking} search for invariant parts of the communities by performing multiple runs of the same algorithm on the same snapshot, Wang et al.\cite{wang2008community} used the concept of Community core nodes, Xu et al. \cite{xu2013analyzing,xu2013community} search for stable community core, Chen et al. \cite{chen2010detecting} use the notion of graph representatives and community representatives, Aynaud et Guillaume \cite{aynaud2010static} proposed a global optimization process in which the modularity is maximized on multiple snapshots rather than one snapshot, Chakrabrti el al. \cite{chakrabarti2006evolutionary} integrate the history cost in their objective function. Methods using deterministic definitions resolve naturally this problem, like k-clique community definition in the CPM method by Palla et al. \cite{palla2007quantifying}.
%Methods in the class of Cross Time approaches don’t suffer from this problem as well, as they consider simultaneously all the network evolution steps.
Community drifting effects: which means that the solution can be dragged away from an originally relevant solution. This problem my affects only temporal trade-off approaches, and more precisely, the updating approaches (see methods in \cite{aynaud2010static, nguyen2011adaptive,aktunc2015dynamic}), when communities at a time $t$ are computed by updating the ones discovered at previous time step $t-1$. Community drift phenomenon arises from the use of non-intrinsic community definitions, i.e., when the community definition depends on the whole network (like modularity), a community can be modified as a result of some changes in an unrelated part of the network, and this could lead to misleading results. It my also occurs when using stochastic community definitions, as partitions evolve based on local optimal solutions, it is not guaranteed to yield an optimal solution at the global level.

\item Most definitions are designed for \textit{disjoint} (non-overlapping) communities, i.e., a node cannot be part of several communities. The ability to detect an overlapping coverage is a crucial question in community detection, especially when exploring real world networks such as social networks. In such networks, nodes are likely belong to multiple communities, in an online social network for example, a member may be connected to co-workers, friends , family,  neighbors, etc. Few method are enable to detect such overlapping community structures, as example: CPM method \cite{palla2007quantifying} which use the concept of maximal k-clique, the method by  ... 
\end{itemize}



%From this review of the literature, we can highlight significant research gaps that still need to be addressed on the topic of dynamic community detection, especially when dealing with social networks. 

As illustrated in Table \ref{tab:meth0}, theses issues are particularly related to the definition of community and to the underling network model used. 

\textbf{\textit{Community definition.}} The existing methodologies propose different definitions of dynamic communities: 
\begin{enumerate}[(i)]
\item Some definitions are \textit{\textbf{stochastic}} and/or \textit{\textbf{extrinsic}}, and thus lead to two major problems:
\begin{itemize}
\item \textbf{\textit{Instability:} }This problem happens when different runs on the same (slightly modified) network lead to very different results. It affects only the two classes of Instant Optimal  approaches and Temporal Trade-off approaches which are based on stochastic and non-deterministic community definitions, like those based on Modularity \cite{asur2009event}, or random walks \cite{tajeuna2015tracking}. Cross time approaches (see methods in \cite{aynaud2011multi, xu2013analyzing, xu2013community, ludkin2018dynamic, jdidia2007communities, mucha2010community}) don't suffer from the instability problem as they propose to study simultaneously all the network evolution steps. Different solutions have been proposed to mitigate this problem: Hopcroft et al. \cite{hopcroft2004tracking} search  for invariant parts of the communities by performing multiple runs of the same algorithm on the same snapshot, Wang et al.\cite{wang2008community} used the concept of Community core nodes, Xu et al. \cite{xu2013analyzing,xu2013community} search for stable community core, Chen et al. \cite{chen2010detecting} use the notion of graph representatives and community representatives, Aynaud and Guillaume \cite{aynaud2010static} propose a global optimization process in which the modularity is maximized on multiple snapshots rather than one snapshot, Chakrabrti el al. \cite{chakrabarti2006evolutionary} integrate the history cost in their objective function. Methods using deterministic definitions resolve naturally this problem, like k-clique community definition in the CPM method by Palla et al. \cite{palla2007quantifying}.
%Methods in the class of Cross Time approaches don’t suffer from this problem as well, as they consider simultaneously all the network evolution steps.
\item \textbf{\textit{Community drifting effects:}} Community drifting means that the solution can be dragged away from an originally relevant solution. This problem might affects only temporal trade-off approaches, and more precisely, the updating approaches (see methods in \cite{aynaud2010static, nguyen2011adaptive,aktunc2015dynamic}), when communities at a time $t$ are computed by updating the ones discovered at previous time step $t-1$. Community drift phenomenon arises from the use of non-intrinsic community definitions, i.e., when the community definition depends on the whole network (like modularity), a community can be modified as a result of some changes in an unrelated part of the network, and this could lead to misleading results. It may also occurs when using stochastic community definitions, as partitions evolve based on local optimal solutions, it is not guaranteed to yield an optimal solution at the global level.
\end{itemize}
\item Most definitions are designed for \textit{\textbf{disjoint}} (non-overlapping) communities, i.e., a node cannot be part of several communities. The ability to detect an overlapping coverage is a crucial question in community detection, especially when exploring real world networks such as social networks. In such networks, nodes are likely belonging to multiple communities, in an online social network for example, a member may be connected to co-workers, friends , family,  neighbors, etc. Few method are enable to detect such overlapping community structures, as example: CPM method \cite{palla2007quantifying} which use the concept of maximal k-clique, the method by  ... 
\end{enumerate}

\textbf{\textit{Network model.}} The way to model the network evolution is extremely important and it highly influence the community detection:

\begin{enumerate}[(i)] 
\item Snapshot models cannot capture the \textit{\textbf{full temporal evolution}} of the networks, and hence methods based on this model (such as )are not suitable to deal with highly evolving networks, which is the case of most real world networks like social networks. On the contrary, temporal network is the appropriate model to deal with \textit{highly evolving networks}, but methods using such a model(like ) are \textit{computationally expensive}, as they require repetitive computations of communities at each network change. Therefore, the majority of recent methods adopts local computations to minimize the computational cost, like the method by Nguyen et al. \cite{nguyen2011adaptive}.   
\item The snapshot model often requires to choose an arbitrary \textit{\textbf{temporal scale}} to divide the network. Communities detected at such an arbitrary temporal granularity could lead to misleading results: communities resulting from high frequency interactions and short duration are invisible when considering large temporal scale (window time), while communities resulting from low frequency interactions and large duration are invisible using a fine temporal granularity. A multiple temporal scale analysis of communities seem therefore the right solution in such a case. To the best of our knowledge, this question has not yet been studied in the literature.
\end{enumerate}
\end{comment}
\subsection{Advantages and drawbacks of dynamic community detection approaches}

This classification highlights a variety of methods which propose different ways for solving the same problem and also different definitions of dynamic communities. %Despite the wide range of definitions and techniques proposed, there are still many 

The proposed taxonomy gives us some hints to choose the appropriate method. The choice depends on the purpose of the analysis. %As mentioned earlier, each classes has its own advantages and disadvantages and each of them is appropriated for a specific use case. 
For example, Instant-optimal approaches are the best choice %when dealing with less evolving networks or 
when the goal is to find communities of high quality at each time step. Temporal trad-off approaches are suitable for the online monitoring and tracking of communities. Finally, the Cross-time approaches are the best choice when the goal is to find coherent communities over a long period of time.



%As mentioned throughout this section, the three classes have their own advantages and disadvantages, and none of these classes is superior to the others. However, some criteria can be also considered while choosing the appropriate approach, like, the network model, instability and community drift problems, the  temporal complexity of the method, etc. 

\subsection{Discussion}\label{chp3:Discussion}

From this review of the literature, we can highlight significant research gaps that still need to be addressed on the topic of dynamic community detection, especially when dealing with social networks. 
To illustrate such problems, we use Table \ref{tab:meth0} which summarizes the comparison between methods of DCD. %The comparison is restricted to only methods designed for detecting overlapping community structures and generic methods which can be applied for both overlapping and  disjoint communities. 
Given the large number of methods being presented in this survey, the comparison is restricted to only some representative methods from each class of approaches. The following comparison criteria are used here:
\begin{itemize}
\item \textit{Approach:} indicates the class of approaches to which the method belongs: \textbf{IO} (Instant Optimal), \textbf{TTO} (Temporal Trade-off) or \textbf{CT} (CrossTime). 
\item Network model: refers to the type of the dynamic network model used by the method: {\textcolor{red}{SN}} (Snapshot Network), {\textcolor{green!80!black}{TN}} (Temporal networks).
\item \textit{Stability:} indicates if the method suffer (\xmark) or not (\cmark) from the Instability problem.
\item \textit{Avalanche safety :} %No community drift
indicates if the method suffer (\xmark) or not (\cmark) from the community drift problem.
\item \textit{Overlapping: }indicates it the method can detect overlapping community structures (\cmark) or not (\xmark).
\item \textit{Multi-temporal scale: }indicates it the method can detect community structures at multiple temporal scale (\cmark) or only on one temporal scale(\xmark).

\end{itemize}


\begin{table}[H]
\resizebox{\textwidth}{!}{%
%\small
\tiny
\begin{tabular}{|p{3.3cm}||p{1.4cm}|p{1.2cm}|p{1.3cm}|p{1.6cm}|p{1.7cm}|p{1.7cm}|}
\hline
\textbf{Reference} & \textbf{Approach}& \textbf{Network Model}& \textbf{Instability}& \textbf{Community drift}& \textbf{Overlapping}& \textbf{Multi-temporal scale} \\ \hline
Asur et al.\cite{asur2009event}& 
\textbf{IO}& 
\textbf{{\textcolor{red}{SN}}}& 
\xmark&
\cmark&
\xmark&
\xmark
\\ \hline
Hopcroft et al.\cite{hopcroft2004tracking}& 
\textbf{IO}& 
\textbf{{\textcolor{red}{SN}}}& 
\cmark&
\cmark&
\xmark&
\xmark
\\ \hline
Palla et al.\cite{palla2007quantifying}& 
\textbf{IO}& 
\textbf{{\textcolor{red}{SN}}}& 
\cmark&
\cmark&
\cmark&
\xmark
\\ \hline
Tajeuna et al.\cite{tajeuna2015tracking}& 
\textbf{IO}& 
\textbf{{\textcolor{red}{SN}}}& 
\xmark&
\cmark&
\xmark&
\xmark
\\ \hline
Wang et al.\cite{wang2008community}& 
\textbf{IO}& 
\textbf{{\textcolor{red}{SN}}}& 
\cmark&
\cmark&
\xmark&
\xmark
\\ \hline
Chen et al.\cite{chen2010detecting}& 
\textbf{IO}& 
\textbf{{\textcolor{red}{SN}}}& 
\cmark&
\cmark&
\xmark&
\xmark
\\ \hline
Aynaud and Guillaume \cite{aynaud2010static}& 
\textbf{TTO}& 
\textbf{{\textcolor{red}{SN}}}& 
\xmark&
\xmark&
\xmark&
\xmark
\\ \hline
Aktunc et al. \cite{aktunc2015dynamic}& 
\textbf{TTO}& 
\textbf{{\textcolor{red}{SN}}}& 
\xmark&
\xmark&
\xmark&
\xmark
\\ \hline
Nguyen et al. \cite{nguyen2011adaptive}& 
\textbf{TTO}& 
\textbf{{\textcolor{green!80!black}{TN}}}& 
\xmark&
\xmark&
\xmark&
\xmark
\\ \hline
Chakraborti et al. \cite{chakrabarti2006evolutionary}& 
\textbf{TTO}& 
\textbf{{\textcolor{red}{SN}}}& 
\cmark&
\xmark&
\xmark&
\xmark
\\ \hline
Xu et al. \cite{xu2013analyzing,xu2013community}& 
\textbf{TTO}& 
{{\textcolor{green!80!black}{TN}}}&%\textbf{{\textcolor{red}{SN}}}& 
\cmark&
\xmark&
\xmark&
\xmark
\\ \hline
Aynaud et Guillaume \cite{aynaud2011multi}& 
\textbf{CT}& 
\textbf{{\textcolor{red}{SN}}}& 
\cmark&
\cmark&
\xmark&
\xmark
\\ \hline
Xu et al. \cite{xu2013analyzing,xu2013community}& 
\textbf{CT}& 
\textbf{{\textcolor{red}{SN}}}& 
\cmark&
\cmark&
\xmark&
\xmark
\\ \hline
Ludkin et al. \cite{ludkin2018dynamic}& 
\textbf{CT}& 
\textbf{{\textcolor{red}{SN}}}& 
\cmark&
\cmark&
\xmark&
\xmark
\\ \hline
Mucha et al. \cite{mucha2010community}& 
\textbf{CT}& 
\textbf{{\textcolor{red}{SN}}}& 
\cmark&
\cmark&
\xmark&
\xmark
\\ \hline
Jdidia et al. \cite{jdidia2007communities}& 
\textbf{CT}& 
\textbf{{\textcolor{red}{SN}}}& 
\cmark&
\cmark&
\xmark&
\xmark
\\ \hline
\textbf{Our $1^{st}$ method \cite{boudebza2018}}& 
\textbf{TTO}& 
\textbf{{\textcolor{green!80!black}{TN}}}& 
\cmark&
\cmark&
\cmark&
\xmark
\\ \hline
\textbf{Our $2^{nd}$  method \cite{boudebza2019detecting}}& 
\textbf{CT}& 
\textbf{{\textcolor{green!80!black}{TN}}}& 
\cmark&
\cmark&
\cmark&
\cmark
\\ \hline
\end{tabular}}
\caption{Comparing dynamic community detection methods.}
\label{tab:meth0}
\end{table}
\begin{comment}
Gauvin et al. \cite{aynaud2011multi}& 
CT& 
{\textcolor{red}{SN}}& 
&
&
\\ \hline
Sarantopolos et al. \cite{sarantopoulos2018timerank}& 
CT& 
{\textcolor{red}{SN}}& 
&
&
\\ \hline
Yan et al. \cite{}& 
CT& 
{\textcolor{red}{SN}}& 
&
&
\\ \hline
\\ \hline
Guo et al. \cite{guo2014evolutionary}& 
TTO& 
{\textcolor{green!80!black}{TN}}& 
\xmark&
\xmark&
\xmark
\begin{itemize}
\item Some definitions are \textit{stochastic} and/or \textit{extrinsic}, and thus lead to two major problems:
Instability : This problem happens when different runs on the same (slightly modified) network lead to very different results. It affects only the two classes of Instant Optimal  approaches and Temporal Trade-off approaches which are based on scholastic and non deterministic community definitions, like those based on Modularity \cite{asur2009event}, or on random walk \cite{tajeuna2015tracking}. Cross time approaches don't suffer from the instability problem as they propose to study simultaneously all the network evolution steps. Diffrent solutions have been proposed to mitigate this problem : Hopcroft et al. \cite{hopcroft2004tracking} search  for invariant parts of the communities by performing multiple runs of the same algorithm on the same snapshot, Wang et al.\cite{wang2008community} used the concept of Community core nodes, Xu et al. \cite{xu2013analyzing,xu2013community} search for stable community core, Chen et al. \cite{chen2010detecting} use the notion of graph representatives and community representatives, Aynaud et Guillaume \cite{aynaud2010static} proposed a global optimization process in which the modularity is maximized on multiple snapshots rather than one snapshot, Chakrabrti el al. \cite{chakrabarti2006evolutionary} integrate the history cost in their objective function. Methods using deterministic definitions resolve naturally this problem, like k-clique community definition in the CPM method by Palla et al. \cite{palla2007quantifying}.
%Methods in the class of Cross Time approaches don’t suffer from this problem as well, as they consider simultaneously all the network evolution steps.
Community drifting effects: which means that the solution can be dragged away from an originally relevant solution. This problem my affects only temporal trade-off approaches, and more precisely, the updating approaches (see methods in \cite{aynaud2010static, nguyen2011adaptive,aktunc2015dynamic}), when communities at a time $t$ are computed by updating the ones discovered at previous time step $t-1$. Community drift phenomenon arises from the use of non-intrinsic community definitions, i.e., when the community definition depends on the whole network (like modularity), a community can be modified as a result of some changes in an unrelated part of the network, and this could lead to misleading results. It my also occurs when using stochastic community definitions, as partitions evolve based on local optimal solutions, it is not guaranteed to yield an optimal solution at the global level.

\item Most definitions are designed for \textit{disjoint} (non-overlapping) communities, i.e., a node cannot be part of several communities. The ability to detect an overlapping coverage is a crucial question in community detection, especially when exploring real world networks such as social networks. In such networks, nodes are likely belong to multiple communities, in an online social network for example, a member may be connected to co-workers, friends , family,  neighbors, etc. Few method are enable to detect such overlapping community structures, as example: CPM method \cite{palla2007quantifying} which use the concept of maximal k-clique, the method by  ... 
\end{itemize}
\end{comment}


%From this review of the literature, we can highlight significant research gaps that still need to be addressed on the topic of dynamic community detection, especially when dealing with social networks. 

As illustrated in Table \ref{tab:meth0}, theses issues are particularly related to the definition of community and to the underling network model used. 

\textbf{\textit{Community definition.}} The existing methodologies propose different definitions of dynamic communities: 
\begin{enumerate}[(i)]
\item Some definitions are \textit{\textbf{stochastic}} and/or \textit{\textbf{extrinsic}}, and thus lead to two major problems:
\begin{itemize}
\item \textbf{\textit{Instability:} }This problem happens when different runs on the same (slightly modified) network lead to very different results. It affects only the two classes of Instant Optimal  approaches and Temporal Trade-off approaches which are based on stochastic and non-deterministic community definitions, like those based on Modularity \cite{asur2009event}, or random walks \cite{tajeuna2015tracking}. Cross time approaches (see methods in \cite{aynaud2011multi, xu2013analyzing, xu2013community, ludkin2018dynamic, jdidia2007communities, mucha2010community}) don't suffer from the instability problem as they propose to study simultaneously all the network evolution steps. Different solutions have been proposed to mitigate this problem: Hopcroft et al. \cite{hopcroft2004tracking} search  for invariant parts of the communities by performing multiple runs of the same algorithm on the same snapshot, Wang et al.\cite{wang2008community} used the concept of Community core nodes, Xu et al. \cite{xu2013analyzing,xu2013community} search for stable community core, Chen et al. \cite{chen2010detecting} use the notion of graph representatives and community representatives, Aynaud and Guillaume \cite{aynaud2010static} propose a global optimization process in which the modularity is maximized on multiple snapshots rather than one snapshot, Chakrabrti el al. \cite{chakrabarti2006evolutionary} integrate the history cost in their objective function. Methods using deterministic definitions resolve naturally this problem, like k-clique community definition in the CPM method by Palla et al. \cite{palla2007quantifying}.
%Methods in the class of Cross Time approaches don’t suffer from this problem as well, as they consider simultaneously all the network evolution steps.
\item \textbf{\textit{Community drifting effects:}} Community drifting means that the solution can be dragged away from an originally relevant solution. This problem might affects only temporal trade-off approaches, and more precisely, the updating approaches (see methods in \cite{aynaud2010static, nguyen2011adaptive,aktunc2015dynamic}), when communities at a time $t$ are computed by updating the ones discovered at previous time step $t-1$. Community drift phenomenon arises from the use of non-intrinsic community definitions, i.e., when the community definition depends on the whole network (like modularity), a community can be modified as a result of some changes in an unrelated part of the network, and this could lead to misleading results. It may also occurs when using stochastic community definitions, as partitions evolve based on local optimal solutions, it is not guaranteed to yield an optimal solution at the global level.
\end{itemize}
\item Most definitions are designed for \textit{\textbf{disjoint}} (non-overlapping) communities, i.e., a node cannot be part of several communities. The ability to detect an overlapping coverage is a crucial question in community detection, especially when exploring real world networks such as social networks. In such networks, nodes are likely belonging to multiple communities, in an online social network for example, a member may be connected to co-workers, friends , family,  neighbors, etc. Few method are enable to detect such overlapping community structures, as example: CPM method \cite{palla2007quantifying} which use the concept of maximal k-clique, the method by  ... 
\end{enumerate}

\textbf{\textit{Network model.}} The way to model the network evolution is extremely important and it highly influence the community detection:

\begin{enumerate}[(i)] 
\item Snapshot models cannot capture the \textit{\textbf{full temporal evolution}} of the networks, and hence methods based on this model (such as )are not suitable to deal with highly evolving networks, which is the case of most real world networks like social networks. On the contrary, temporal network is the appropriate model to deal with \textit{highly evolving networks}, but methods using such a model(like ) are \textit{computationally expensive}, as they require repetitive computations of communities at each network change. Therefore, the majority of recent methods adopts local computations to minimize the computational cost, like the method by Nguyen et al. \cite{nguyen2011adaptive}.   
\item The snapshot model often requires to choose an arbitrary \textit{\textbf{temporal scale}} to divide the network. Communities detected at such an arbitrary temporal granularity could lead to misleading results: communities resulting from high frequency interactions and short duration are invisible when considering large temporal scale (window time), while communities resulting from low frequency interactions and large duration are invisible using a fine temporal granularity. A multiple temporal scale analysis of communities seem therefore the right solution in such a case. To the best of our knowledge, this question has not yet been studied in the literature.
\end{enumerate}
\end{comment}
